How Well Can General Vision-Language Models Learn Medicine By Watching Public Educational Videos?

Publicly available biomedical videos, such as those on YouTube, serve as valuable educational resources for medical students. Unlike standard machine learning datasets, these videos are designed for human learners, often mixing medical imagery with narration, explanatory diagrams, and contextual framing. In this work, we investigate whether such pedagogically rich, yet non-standardized and heterogeneous videos can effectively teach general-domain vision-language models biomedical knowledge. To this end, we introduce OpenBiomedVi, a biomedical video instruction tuning dataset comprising 1031 hours of video-caption and Q/A pairs, curated through a multi-step human-in-the-loop pipeline. Diverse biomedical video datasets are rare, and OpenBiomedVid fills an important gap by providing instruction-style supervision grounded in real-world educational content. Surprisingly, despite the informal and heterogeneous nature of these videos, the fine-tuned Qwen-2-VL models exhibit substantial performance improvements across most benchmarks. The 2B model achieves gains of 98.7% on video tasks, 71.2% on image tasks, and 0.2% on text tasks. The 7B model shows improvements of 37.09% on video and 11.2% on image tasks, with a slight degradation of 2.7% on text tasks compared to their respective base models. To address the lack of standardized biomedical video evaluation datasets, we also introduce two new expert curated benchmarks, MIMICEchoQA and SurgeryVideoQA. On these benchmarks, the 2B model achieves gains of 99.1% and 98.1%, while the 7B model shows gains of 22.5% and 52.1%, respectively, demonstrating the models' ability to generalize and perform biomedical video understanding on cleaner and more standardized datasets than those seen during training. These results suggest that educational videos created for human learning offer a surprisingly effective training signal for biomedical VLMs.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace with \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction clearly state the claims and main contributions of the paper, which include evaluating general-purpose VLMs for biomedical video analysis and proposing a new biomedical video instruction-tuning dataset along with standardized evaluation benchmarks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include a dedicated paragraph at the end of the Discussion and Conclusion section that addresses limitations, such as potential LLM hallucinations and the scope of our evaluation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not have any theoretical results. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we provide detailed descriptions of all hyperparameters, datasets, and model architectures used in the study.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include the code as part of the supplementary material and publicly release all datasets used in the study.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper includes all training and testing details, including data splits, hyperparameters, and types of optimizers used.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper currently does not include error bars. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides details about the compute resources used, including memory requirements, execution time, and other relevant metrics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper complies with all aspects of the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The broader impact of our work is discussed in the Discussion and Conclusion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we include an Ethics Statement following the Conclusion section that addresses these considerations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we have properly credited the parent datasets. Both the code and data will be open-sourced and made freely available for research purposes.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we provide detailed information about our fine-tuning and evaluation datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: None of the datasets used in this work contain any PHI or sensitive information. We also do not work directly with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: IRB approval is not required for this study, as we do not work with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: An LLM was not used in writing this paper; therefore, this item is not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sec/scratch.tex <==
\begin{abstract}

Access to clean biomedical videos are restricted to academic institutions. Youtube has been a great source of education materials, where there are hundreds of hours of free biomedical education videos. Medical students spend countless hours watching these education videos, as part of their training. We were curious to understand if a general domain large vision-language model can also learn medicine by watching these relatively noisy and educational biomedical videos. In this paper, we curate over 1000 hours of biomedical video-caption dataset. Through human-ai collaboration, we clean the dataset through multi-step cleaning pipeline, with both human and AI involved throughout multiple steps, to reach to 230 hours of biomedical video-caption finetuning dataset. Along with caption, we generated multi-turn Q/A style instruction following dataset and finetuned Qwen-2-VL series of models. We evaluate the models medical understanding using three sets of benchmark tasks: text-only benchmarks, image-text benchmarks, and video-text benchmarks. We observe that by watching hundreds of hours of publicly available biomedical youtube videos, these models domain models can adapt pretty well to a range of relevant biomedical tasks, achieving 3.4\% improvement on text, 45.8\% on image, and 12.5\% on video on 2B model, and 2.9\% on image, 35.2\% on image, and 7.5\% improvement on 7B model class over base model. 


One of the difficulty of the field is the lack of standaridized biomedical video evaluation dataset. There are plenty of such benchmarks on text-only, and image-text space. Therefore, as a by-product of our work, we also curate two biomedical video understanding evaluation datasets, called MIMICEchoQA, and SurgicalVideoQA. We release our finetuned models, codebase, as well as finetuning and evaluation dataset for community to further clean and evaluate biomedical vision models. 

230 hours of biomedical video-caption dataset. 

Large Multimodal models have shown impressive abilities in solving various general domain tasks, including their adoption to domain specific fields such as medicine. While their adoption in the f


Motivated by the current adoption of large foundation models on biomedical domain, we set to explore the video-language models in the biomedical domain. However, currently, there isn't a large scale biomedical video, focused on medical diagnosis, disease pathology, and medical procedures, available in public domain for easy use. Motivated by this challenge, we curated a 


We investigate whether open-domain vision-language models can acquire essential biomedical vision concepts by learning from publicly available educational biomedical videos. Large-scale, publicly available biomedical video datasets for model training are scarce, with most being closed-source or too small, task-specific, and unrelated to medical diagnosis, disease pathology, and human anatomy. To address this gap, we curated [TODO: Dataset Name], a dataset comprising [TODO: XX] hours of biomedical videos from YouTube, using a human-AI collaborative approach for cleaning and processing. We fine-tuned Qwen-2-VL series of models (2B, 7B) on this dataset and introduced [TODO: Benchmark Name], a benchmark derived from our dataset to assess model performance under a similar distribution. Since both our dataset and benchmark consist of noisy educational biomedical videos, we also evaluated the models on a set of publicly available, high-quality biomedical video and image benchmarks to assess their generalization. We release [TODO: Dataset Name] and [TODO: Benchmark Name] to support future research in biomedical vision-language learning. Our findings [TODO: summarize key results], highlighting the potential of self-supervised learning from publicly available biomedical resources.
\end{abstract}


\subsection{Data Processing}
\label{subsection_data_processing}

From 12000 raw videos what we got from the data curation step, not all videos were clean or even relevant. In order to clean our dataset, we used a multi-step cleaning process, involving AI and human working together. 

For our first step, we annotated 16.9K example frames from our entire data distribution (all frames from all raw videos) using GPT-4o mini to classify them as biomedical or non-biomedical frames. The prompt used for classification (detailed in Appendix \ref{subsubsection_medical_image_prompt}) was carefully engineered through human iteration to ensure accurate labeling. We specifically designed the prompt to identify frames containing predominantly visual biomedical features (e.g., medical scans, surgical procedures, anatomical visualizations), while explicitly excluding frames that only contained biomedical text or showed medical professionals without accompanying medical imagery. This design choice was intentional, as our goal was to build a dataset focused on learning from medical visual content rather than text-based information. A human annotator also independently labeled 1000 of these frames, and the agreement between GPT-4o mini and human was 95.0\%, further adding confidence to this step. 

In our second step, we leveraged the GPT labeled data to fine-tune a SigLIP model with an added image classification head. Specifically, we used \texttt{siglip-base-patch16-224}. The model was fine-tuned for 3 epochs on 8 H100 GPUs using a per-device batch size of 32, learning rate of 2e-5, and weight decay of 0.01. To validate our approach, we evaluated our fine-tuned model, \texttt{siglip-medical}, on a benchmark of 487 human-annotated medical images, achieving a high concordance of 95.48\% with human labels.

In our third step, we extracted audio from all videos and processed it using  \texttt{Whisper-large-v3} model to generate transcriptions. For videos containing non-English audio, the model automatically translated the content into English during transcription.

In our fourth step, we used \texttt{siglip-medical} to segment videos into biomedical and non-biomedical sections. We processed each video by classifying frames at 0.5-second intervals, obtaining biomedical probability scores for each frame. Our segmentation algorithm (detailed in Appendix \ref{subsection_segmentation_algorithm}) was designed to be comprehensive in capturing biomedical content while being tolerant of brief interruptions. Specifically, we implemented a greedy approach that identified continuous segments of biomedical frames while allowing gaps of up to 10 non-biomedical frames between them. These gaps were then stitched together to form coherent segments. Finally, we paired these extracted biomedical video segments with their corresponding transcriptions from Whisper to create our video-caption pairs.
    
In our fifth step, we implemented an additional filtration layer using GPT-4 to ensure the captions were biomedically relevant. We designed a prompt (detailed in Appendix \ref{subsubsection_caption_filtering}) that specifically identifies captions describing observable biomedical content in videos while excluding irrelevant, incomplete, or purely textual information (information that does not discuss predominant information in videos). The prompt was engineered to retain captions that describe visual biomedical elements (such as procedures, diagnosis, or anatomical demonstrations) while filtering out captions that were too short, ambiguous, or lacked specific biomedical context. This filtration process resulted in approximately 4.5K relevant biomedical videos. This step helped maintain the quality and relevance of our dataset by ensuring all retained captions had meaningful biomedical content that could be visually observed in the corresponding video segments.
    
In our sixth step, we conducted a thorough manual review of the 4.5K videos, dividing them into finetuning dataset, and in-domain evaluation dataset. The evaluation dataset only comprises of surgical videos, as that is one major video modality that is lacking evaluation benchmarks in public domain, tailored towards vision-language model undersanding. The existing surgical benchmarks are largly focused on classification models or identifying tools and specific scenes from static surgical frames. We descrive this SurgicalVideoQA dataset in more detail in ~\ref{subsection_benchmark_design}. 

In our seventh step, we enhanced caption quality across both fine-tuning and benchmark datasets using GPT-4o. We developed a prompt (detailed in Appendix \ref{subsubsection_caption_cleaning}) that instructs the model to clean and standardize captions while maintaining strict adherence to the original content. The prompt was designed to achieve several key objectives: standardizing biomedical terminology, maintaining appropriate detail levels, preserving explicit spatial and temporal context, removing non-visual information unless contextually essential, and ensuring neutral, objective language. This cleaning process transformed potentially colloquial or inconsistent captions into clear, descriptive text.

In our eighth step, we leveraged GPT-4o to generate comprehensive question-answer pairs and structured metadata from the cleaned captions (prompt detailed in Appendix \ref{subsubsection_qa_metadata}). The Q/A generation was designed to create diverse question types, including hierarchical questions (from general to detailed), temporal and sequential questions, complex reasoning questions, and varied question forms (why, how, compare). For metadata extraction, we systematically captured eight key categories: biomedical modality (e.g., X-ray, MRI), pathologies and conditions, anatomical regions, procedure types, tools and equipment, temporal context, environmental setting, and roles and actions. This structured approach ensured consistent annotation across our dataset while maintaining strict grounding in the caption content and appropriately handling ambiguous cases.


\paragraph{Image Benchmarks}

For the image understanding, we picked three common benchmarks: PathVQA [cite, link: https://huggingface.co/datasets/flaviagiammarino/path-vqa], RadVQA [cite, link: https://huggingface.co/datasets/flaviagiammarino/vqa-rad], and Slake [cite, link: https://www.med-vqa.com/slake/]. PathVQA is ... RadVQA is ..., and Slake is ...

We focused on the closed ended question evaluation, and accessed the performance using accuracy. Second figure in Figure~\ref{fig:multimodal_benchmarks} presents performance comparison on image benchmarks. Here, we see relatively much more performance improvement than text benchmark. 

On RadVQA, we see 1240\% improvement over baseline on Qwen-2-VL-2B
178.8\% on Qwen-2-VL-7B

On PVQA, 3571\% improvement  over baseline on Qwen-2-VL-2B
198.2\% on Qwen-2-VL-7B

On Slake, 111.1\% over baseline on Qwen-2-VL-2B
31.2\% over baseline on Qwen-2-VL-7B


Slake dataset provides with modality information for each images. We further used GPT-4o, given the image and question/answer, to generata image modlaity for radvqa dataset as well. And we combined these two datasets to stratify the model performance across different image modality. This is interesting to look at, in light of our finetuning data statistics, shown in Figure~\ref{fig:finetuning_dataset_statistics}. CT (7.8 hours), MRI (7.8 hours), X-ray (2.4 hours). Firstly, across all modalities, finetuned models outperform baseline models significantly. Second, we see that models perform the best for both 2B and 7B models. Interestingly, closely followed by CT, which makes sense because we have 7.8 hours of these modalities. Interestingly, model performance on X-ray is not far behind either, even though there was only 2.4 hours of training dataset for that modality. The performance gain must have come from our finetuning dataset, as the base model performance is much worse. 

X-Ray: 763.2\% on 2B model; 150.9\% on 7B
CT: 157.9\% on 2B model; 34\% on 7B
MRI: 133.2\% on 2B model; 89.3\% on 7B model. 



we leveraged the modality labels provided in Slake and used \texttt{GPT-4o} to generate similar modality labels for RadVQA. This allowed us to stratify results based on modality and compare them against our fine-tuning dataset statistics in Figure~\ref{fig:finetuning_dataset_statistics}, where CT and MRI images account for 7.8 hours each, while X-ray images account for only 2.4 hours. Across all imaging modalities, fine-tuned models significantly outperformed their respective baselines. The highest accuracy was achieved on MRI images, closely followed by CT scans, which aligns with the distribution of our training data. Interestingly, despite having only 2.4 hours of X-ray training data, the model performed competitively, suggesting that fine-tuning contributed substantially to its improvement over the base model.

On X-ray images, the \texttt{Qwen-2-VL-2B} model improved by 763.2\%, while the \texttt{Qwen-2-VL-7B} model improved by 150.9\%. On CT scans, the \texttt{Qwen-2-VL-2B} model achieved a 157.9\% gain, while the \texttt{Qwen-2-VL-7B} model improved by 34\%. On MRI images, the \texttt{Qwen-2-VL-2B} model improved by 133.2\%, while the \texttt{Qwen-2-VL-7B} model achieved an 89.3\% gain. The results is shown in \cref{fig:modality_accuracies}


On text-only benchmarks, we observe that training on captions alone provides a moderate boost in performance. On MedQA, the text-only model achieves 52.6\% accuracy, while the fully fine-tuned model achieves 56.2\%, a modest 6.8\% improvement. Similarly, on PubMedQA, the text-only model scores 73.8\%, while the full model reaches 76.0\%, a 3.0\% increase. These results suggest that training on biomedical video captions alone contributes meaningfully to textual reasoning but offers limited additional gains beyond the base model.

For image-based tasks, the fully fine-tuned model substantially outperforms the text-only model, reinforcing the importance of visual grounding. On RadVQA, the text-only model achieves only 26.3\%, whereas the full model reaches 73.3\%, marking a 178.7\% relative improvement. Similarly, on PathVQA, the text-only model scores 21.7\%, compared to 64.7\% for the full model, resulting in a 198.2\% increase. On Slake, the text-only model achieves 50.7\%, while the fully fine-tuned model improves to 66.5\%. These results indicate that while captions provide useful textual knowledge, they lack the critical visual information necessary for medical image interpretation.


\subsection{Ablation Studies}
\label{subsection_ablation_studies}

To better understand the contributions of different components of our dataset, we conducted several ablation studies. All models were trained using the same configuration as our main fine-tuned models (Table~\ref{tab:training_config}), ensuring a direct and fair comparison.

\paragraph{Text-Only Training.}  
To isolate the effect of video-text alignment, we trained \texttt{Qwen-2-VL-7B-Instruct} model using only the text extracted from videos, without the accompanying video frames. This experiment allows us to disentangle the improvements gained from video-text pairs compared to training on biomedical text alone. During evaluation time, all models were evaluated with both image/video and text. \cref{fig:multimodal_benchmarks_text_only_7B_models} presents the result of this ablation. On text benchmarks, we observe that training on biomedical text along from the videos provides a moderate boost in performance, showing that training on biomedical video captions alone contributes meaningfully to textual reasoning but offers limited additional gains beyond the base model.

For image benchmarks, even the model that is trained on just biomedical video captions and Q/A pairs perform significantly better than the base \texttt{Qwen2-VL-7B-Instruct} model. The performance improvement from model trained on text only to fully-finetuned model is modest for RaqVQA and Slake, however, on PathVQA, the performance difference is significant with 64.5\% improvement over the text-only finetuned model. One main reason why this could be happening is because, even though the model finetuned on biomedical video captions and Q/A pairs, it still has seen more biomedical context and Q/A pairs similar to what it would be seeing in the image benchmarks. Nonetheless, these results indicate that while captions provide useful textual knowledge, they lack the critical visual information necessary for medical image interpretation.

On video benchmarks, we see the largest gap, where fine-tuning on both video and text significantly enhances performance. On \mimicqa, the text-only model achieves 20.4\% accuracy, whereas the fully fine-tuned model reaches 36.0\%, a 76.5\% improvement. Similarly, on \surgeryqa, the text-only model scores 15.7\%, while the fully fine-tuned model achieves 21.9\%, marking a 39.5\% increase. These findings suggest that textual captions alone fail to capture the temporal and spatial dynamics required for biomedical video understanding.

Overall, this ablation study highlights that while text-only training provides some domain-specific knowledge, and consequently, we see performance improvement from base \texttt{Qwen2-VL-7B-Instruct} model. However, incorporating visual information is essential for achieving strong performance, particularly for image and video tasks.


\paragraph{Data Scaling Analysis.}  
To analyze the impact of increasing training data, we evaluated model performance across different percentages of the dataset and averaged results across text, image, and video benchmarks. Figure~\ref{fig:checkpoint_performance_averaged} presents these trends.

For text-only benchmarks, scaling the dataset results in only marginal performance gains. The \texttt{Qwen-2-VL-7B-biomed} model remains relatively stable across different dataset sizes, suggesting that additional biomedical video-caption data does not significantly enhance performance on purely textual tasks. Note that the size of the caption dataset is much lower than the usual textual data finetuning. Therefore, our entire dataset on itself is pretty low dataset size, compared to other large finetuning dataset, and it may be the artifact of that. 

In contrast, both image and video benchmarks exhibit a clear upward trend with increasing training data, highlighting the importance of dataset size for multimodal understanding. For image benchmarks, performance steadily improves as more data is used, with the largest gains occurring between 25\% and 50\%, after which improvements continue at a slower pace. This suggests that models benefit from a greater diversity of medical images and their associated captions, reinforcing the value of scaling up biomedical multimodal datasets.

The most significant scaling effect is seen in video-based benchmarks, where model performance steadily increases with more data. This trend highlights that video-based tasks, which require both temporal and spatial reasoning, benefit significantly from additional training examples. Notably, while the \texttt{Qwen-2-VL-2B-biomed} model plateaus slightly after 75\% of the dataset, the \texttt{Qwen-2-VL-7B-biomed} model continues to improve, indicating that larger models can better utilize increased data for video understanding.

Overall, these results suggest that while textual benchmarks saturate early, image and video understanding continues to improve with additional data, reinforcing the importance of large-scale multimodal training. The strong data-scaling trend in video benchmarks indicates that further improvements may be possible with even larger and more diverse biomedical video datasets.

\section{Introduction}
\label{sec:intro}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/figures/dataset_pipeline.pdf}
    \caption{End-to-end pipeline for generating our biomedical video fine-tuning and evaluation datasets. The process begins with curating videos from YouTube, followed by multiple steps of filtering and cleaning, including biomedical frame segmentation using SigLip and caption refinement and Q/A generation using GPT-4o. Human verification is integrated at multiple stages throughout the pipeline to ensure data quality.}
    \label{fig:dataset_pipeline}
\end{figure*}


Vision-language models (VLMs) have made significant progress in integrating visual and textual modalities, achieving strong performance in tasks such as image captioning, visual question answering, and multimodal reasoning~\cite{liu2023visual,meta2024llama,hurst2024gpt,beyer2024paligemma,wang2024qwen2,team2024gemini,wang2025cogvlm}. Recent advancements in video-language models have further extended these capabilities to dynamic visual data, enabling the understanding of temporal dependencies in videos and allowing models to respond effectively to natural language queries~\cite{beyer2024paligemma,wang2024qwen2,team2024gemini}. These developments hold significant potential across various domains, including education, entertainment, and healthcare. 

In the biomedical domain, there is growing interest in applying vision-language models to tasks such as medical report generation, disease classification, and procedural video understanding~\cite{saab2024capabilities,thapa2024dragonfly,tu2024towards,li2023llava}. Less explored in biomedical video doamin ... WHy is it important?... Why is it less explored? Probably because of lack of biomedical video dataset in public domain to finetune. Similarly, there is also lack of biomedical video evaluation datasets, hindering progress in this domain ...

Although there has been an increasing number of publicly available biomedical image datasets for vision-language research, biomedical video datasets remain limited in both scale and diversity. Existing biomedical video datasets primarily focus on specific tasks. MedVidQA~\cite{gupta2023dataset} is designed for question-answering on medical instructional videos, while NurViD~\cite{hu2023nurvid} focuses on nursing procedures. Other datasets, such as AVOS~\cite{goodman2024analyzing}, provide surgical videos with metadata annotations but do not cover general biomedical education or instruction tuning dataset or vision-language model evaluation dataset. MIMIC-IV-ECHO~\cite{gow2023mimic} is restricted to echocardiography, and the EndoVis Challenge~\cite{nwoye2023cholectriplet2022} datasets primarily support surgical tool segmentation and phase recognition. While these datasets are valuable for their respective applications, there is no publicly available large-scale biomedical video dataset that covers a diverse set of educational biomedical concepts, such as human anatomy, disease pathology, medical procedures, and clinical diagnostics.  

Additionally, in recent years, YouTube has emerged as an accessible platform for medical students to study medicine~\cite{osman2022youtube, akakpo2024recognizing, chen2019estimating, derakhshan2019assessing, rapp2016youtube}...

However, a critical challenge remains: can open-domain vision-language models learn meaningful biomedical vision concepts from publicly available educational biomedical videos? Answering this question is essential for assessing the feasibility of leveraging freely accessible video data to enhance biomedical AI systems.  

To address this gap, we curate \dataset, a large-scale dataset of 230 hours of publicly available biomedical educational videos from YouTube throug a multi-step human-AI collaborative data curation, filtering, and cleaning processes. Our dataset spans multiple biomedical domains such as ..., and anatomical regions such as ...


and is processed using a human-AI collaborative approach to ensure high-quality structured data. 

To evaluate whether general-domain open-source models can learn biomedical vision concepts from our dataset, we fine-tune multiple scales of Qwen-2-VL models and introduce two biomedical video benchmarks, \surgeryqa and \mimicqa, focused on evaluating biomedical video understandings through open-ended Q/A pairs... \surgeryqa consists of ..., \mimicqa consists of ...

Using this dataset, we finetune \texttt{Qwen-2-VL-2B-Insturct} and \texttt{Qwen-2-VL-7B-Insturct} models and show that ...

Our contributions are as follows:  

\begin{enumerate}
    \item \textbf{Biomedical Video Model Evaluation}: We systematically evaluate the domain adaptaively capabilities of general domain vision-language models to video understanding, to understand if these general domain vision-language models can understand medicine by ``studying'' hours of noisy educational YouTube videos. We show that across text, image, and video benchmarks, ...
    \item \textbf{Biomedical video instruction dataset}: We introduce [TODO: Dataset Name], a large-scale, publicly available dataset of biomedical educational videos, curated from online sources with a structured cleaning process.
    \item \textbf{Biomedical video benchmarks}: We propose [TODO: Benchmark Name], a benchmark for evaluating biomedical video-language models on instructional video understanding.
    \item \textbf{Fine-tuned biomedical vision-language model}: We fine-tune open-domain models on our dataset and assess their ability to learn biomedical vision concepts, comparing performance across multiple external benchmarks.
\end{enumerate}  


% \section{Related Work}
% \label{sec:related_work}

\subsection{Vision Language Models}
describe both imag-text model, and video models

\subsection{Biomedical Vision Language Models}

both biomedical image and text, and video models

\subsection{Biomedical Video Models and Datasets}

Biomedical video analysis has seen significant advancements, supported by various publicly available datasets and benchmarks that facilitate research in this domain. These resources encompass a range of medical procedures and applications, providing valuable data for developing and evaluating algorithms. The MedVidQA dataset (Link: \url{https://medvidqa.github.io/}) focuses on medical video question answering and comprehension, offering a collection of educational biomedical videos to support natural language processing and video analysis in the medical field. NurViD (Link: \url{https://arxiv.org/abs/2310.13347}) is a comprehensive video database designed for nursing procedure activity understanding, including over 1,500 videos covering 51 distinct nursing procedures and 177 action steps, serving as a resource for analyzing clinical workflows and procedural training. The AVOS (Annotated Videos of Open Surgery) dataset (Link: \url{https://research.bidmc.org/surgical-informatics/avos}) comprises 1,997 open surgical videos, each annotated with relevant United Medical Language System (UMLS) tags. This diverse collection, sourced from over 50 countries, supports research in surgical video analysis and object segmentation. MIMIC-IV-ECHO (Link: \url{https://physionet.org/content/mimic-iv-echo/0.1/}) is a module of the MIMIC-IV database, containing a subset of echocardiograms recorded between 2017 and 2019. These echocardiograms are linked to corresponding patient data, providing a resource for cardiac function analysis and diagnostic imaging research. The EndoNet architecture (Link: \url{https://arxiv.org/abs/1602.03012}) is designed for recognition tasks on laparoscopic videos, specifically phase recognition and tool presence detection. Trained on a dataset of 80 cholecystectomy videos, EndoNet demonstrates the application of deep learning in surgical workflow analysis. The Endoscopic Vision (EndoVis) Challenge (Link: \url{https://opencas.dkfz.de/endovis/datasetspublications/}) provides datasets for comparative validation of endoscopic vision algorithms, focusing on various problems each year. These challenges promote advancements in the field by offering data for tasks such as instrument segmentation and surgical workflow analysis. Cataract-1K (Link: \url{https://klausschoeffmann.com/datasets}) is a dataset comprising 1,000 cataract surgery videos, with annotations for surgical phases and instrument usage. This resource supports research in ophthalmic surgery analysis and skill assessment. The Gait Abnormality in Video Dataset (GAVD) (Link: \url{https://arxiv.org/abs/2407.04190}) includes 1,874 video sequences of normal, abnormal, and pathological gaits. Clinically annotated, GAVD facilitates research in computer vision-based gait analysis and biomechanics. BlanketSet (Link: \url{https://arxiv.org/abs/2210.03600}) is an RGB-IR-D action recognition dataset capturing sequences performed in a hospital bed. It addresses the need for public datasets representative of clinical in-bed scenarios, aiding the development of algorithms for patient monitoring and activity recognition. These datasets collectively provide a foundation for advancing biomedical video analysis, enabling the development of algorithms that enhance medical education, surgical procedures, diagnostic processes, and patient care.
